Integral Line-of-Sight Curved Path Following of Helical Microswimmers Actuated by Rotating Magnetic Dipoles

This short paper investigates the problem of curved path following for helical microswimmers actuated by rotating magnetic dipoles. The proposed solution, which relies on an integral line-of-sight (ILOS) guidance law, can be utilized in both below and beyond step-out frequency regimes.

==> section/CLFQP.tex <==
\section{CLF-based Quadratic Program Solution}

\begin{itemize}
	\item This is the trivial solution after the zero dynamics analysis 
	is done. However, it lacks a proper geometric insight. Indeed, this control 
	strategy makes the robot to converge to the zero dynamics manifold in a direction perpendicular 
	to the manifold.  
\end{itemize}

==> section/zerodyn.tex <==



